Force and torque acting on particles in a transitionally rough open channel flow

Direct numerical simulation of open channel flow over a geometrically rough wall has been performed at a bulk Reynolds number of approximately 2900. The wall consisted of a layer of spheres in a square arrangement. Two cases have been considered. In the first case the spheres are small (with diameter equivalent to 10.7 wall units) and the limit of the hydraulically smooth flow regime is approached. In the second case the spheres are more than three times larger (49.3 wall units) and the flow is in the transitionally rough flow regime. Special emphasis is given on the characterisation of the force and torque acting on a particle due to the turbulent flow. It is found that in both cases the mean drag, lift and spanwise torque are to a large extent produced at the top region of the particle surface. The intensity of the particle force fluctuations is significantly larger in the large-sphere case, while the trend differs for the fluctuations of the individual components of the torque. A simplified model is used to show that the torque fluctuations might be explained by the spheres acting as a filter with respect to the size of the flow scales which can effectively generate torque fluctuations. Fluctuations of both force and torque are found to exhibit strongly non-Gaussian probability density functions with particularly long tails, an effect which is more pronounced in the small-sphere case. Some implications of the present results for sediment erosion are briefly discussed.

==> keywords.tex <==
\begin{keywords}
turbulence, rough wall, particle forces, immersed boundary, direct
numerical simulation
\end{keywords}
 

